A Context-Oriented Extension of F#

Context-Oriented programming languages provide us with primitive constructs to adapt program behaviour depending on the evolution of their operational environment, namely the context. In previous work we proposed ML_CoDa, a context-oriented language with two-components: a declarative constituent for programming the context and a functional one for computing. This paper describes the implementation of ML_CoDa as an extension of F#.

==> eptcsdata.tex <==
\providecommand{\firstpage}{18}
\providecommand{\publicationstatus}{Jos\'{e} Proen\c{c}a and Massimo Tivoli (Eds.):\\
14th International Workshop on Foundations of\\
Coordination Languages and Self-Adaptive Systems (FOCLASA'15)\\
EPTCS 201, 2015, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.201.2}{10.4204/EPTCS.201.2}}
\pdfoutput=1

